Trend correlation inference in time series via differencing

How strongly do latent trends move together when we observe only one noisy multivariate time series? This paper addresses this issue by introducing trend correlation, which serves as a measure of structural association. Formal statistical tests, including tests for one-pair, two-pair, and all-pair trend correlation, are proposed via a differencing approach. The resulting test statistic is computationally fast and straightforward as it bypasses direct estimation of the unknown trends and change point estimations. As a natural consequence, we also obtain new tests on trend stationarity in multivariate time series based on trend variance and trend covariance. The developed difference-based trend tests offer the advantage of being sensitive to small oscillating trend effects. Finally, the proposed trend correlation test is applied to study the association between different crime frequencies and weather-related variables in the City of Chicago. The differences between trend correlation and traditional Pearson correlation are revealed, suggesting a new angle for performing criminological analysis.

==> myPreliminary.tex <==
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Packages 
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{varioref} 
\usepackage{xr-hyper} 
\usepackage[colorlinks]{hyperref}
\hypersetup{citecolor=blue}
\hypersetup{linkcolor=red}
\usepackage{booktabs}
\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amsmath}
\usepackage{epsfig,amsmath,amssymb,euscript,amsfonts,hyperref}
\usepackage{natbib}		% ref number 
\usepackage{array}
\usepackage{nccbbb}
\usepackage{verbatim} % for multi-line comments
\usepackage[lined,boxed,commentsnumbered, ruled]{algorithm2e} 
\usepackage{graphicx}
\usepackage{bm}
\usepackage{bbm}	%% \mathbb{1}
\usepackage{dsfont} %% \mathbb{1}
\usepackage{MnSymbol} %% \udots
\usepackage{enumitem}
\usepackage{color}
\usepackage{caption,setspace}						% caption 
\captionsetup{font={small,stretch=1},labelfont=bf} 	% caption setup
\usepackage{lipsum}
\definecolor{darkgreen}{rgb}{0, .6, 0}
\usepackage{multirow}
\usepackage[cal=boondox]{mathalfa}
\usepackage{authblk}
\usepackage{bbold}
\usepackage{subcaption}


%% Tables fixed width
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}  % delete colume of a table 

\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\topfraction}{0.95}
%\renewcommand{\bottomfraction}{0.9}
\renewcommand{\textfraction}{0.05}

%% loose version 
\setlength{\oddsidemargin}{0.15in}
\setlength{\textwidth}{6.2in}
\setlength{\textheight}{8.5in}
\setlength{\topmargin}{-0.35in}
\renewcommand{\baselinestretch}{1.5}

%% dense version 
%\setlength{\oddsidemargin}{-.4in}
%\setlength{\textwidth}{7.3in}
%\setlength{\textheight}{9.75in}
%\setlength{\topmargin}{-0.98in}
%\renewcommand{\baselinestretch}{1.81}

%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Margins
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\renewcommand{\floatpagefraction}{0.9}
\renewcommand{\topfraction}{0.95}
%%%%%\renewcommand{\bottomfraction}{0.9}
\renewcommand{\textfraction}{0.05}

%\addtolength{\oddsidemargin}{-.5in}%
%\addtolength{\evensidemargin}{-.5in}%
%\addtolength{\textwidth}{1in}%
%\addtolength{\textheight}{1.3in}%
%\addtolength{\topmargin}{-.8in}%

%% loose version 
\setlength{\oddsidemargin}{0.15in}
\setlength{\textwidth}{6.2in}
\setlength{\textheight}{8.5in}
\setlength{\topmargin}{-0.35in}
\renewcommand{\baselinestretch}{1.5}

\def\spacingset#1{\renewcommand{\baselinestretch}%
{#1}\small\normalsize} \spacingset{1}

	
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Theorem Style
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
%\startlocaldefs
%\numberwithin{equation}{section}   
%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}

\theoremstyle{definition}
\newtheorem{example}{Example}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{model}{Model}[section]
%\endlocaldefs

\hypersetup{citecolor=myblue}
\hypersetup{linkcolor=myblue}


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### color
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
%\usepackage{xcolor}
\definecolor{BUred}{rgb}{0.8, 0.0, 0.0}
\definecolor{BLUE}{rgb}{0.0, 0.28, 0.67}
\definecolor{magenta}{rgb}{1,0,.6}
\definecolor{blue0}{rgb}{0.95, 0.97, 1.0}
\definecolor{brown}{rgb}{0.75, 0.25, 0.0}
\definecolor{mygreen}{rgb}{0.1, 0.5, 0.1}
\definecolor{myred}{rgb}{0.7, 0.1, 0.1}
\definecolor{myblue}{rgb}{0.1, 0.1, 0.7}
\definecolor{mygold}{rgb}{0.95, 0.85, 0.37}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{myorange}{rgb}{1,0.5,0}


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### Operators 
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\newcommand{\pr}{\mathsf{P}} 
\newcommand{\E}{\mathsf{E}} 
\newcommand{\median}{\mathop{\mathsf{median}}}
\newcommand{\Cov}{{\mathsf{Cov}}} 
\newcommand{\Corr}{{\mathsf{Corr}}} 
\newcommand{\Var}{{\mathsf{Var}}}
\newcommand{\Avar}{{\mathsf{AVar}}}
\newcommand{\Acov}{{\mathsf{ACov}}}
% Only for Biometrika
%\newcommand{\cov}{\mathrm{cov}}
%\newcommand{\var}{\mathrm{var}}
% End
%\newcommand{\Med}{{\mathsf{Med}}}
\newcommand{\CRLB}{{\mathsf{CRLB}}}
\newcommand{\SD}{{\mathsf{SD}}}
\newcommand{\CV}{{\mathsf{CV}}}
\newcommand{\Bias}{{\mathsf{Bias}}}
\newcommand{\AMSE}{\operatorname{\mathsf{AMSE}}}
\newcommand{\MSE}{\operatorname{\mathsf{MSE}}}
\newcommand{\lik}{L} 
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\AIC}{\mathrm{AIC}}
\newcommand{\BIC}{\mathrm{BIC}}
\newcommand{\ARE}{\mathsf{ARE}}
\newcommand{\AV}{\mathsf{AV}}
\newcommand{\AEff}{\mathsf{AE}}
\newcommand{\Eff}{\mathsf{Eff}}
\newcommand{\CP}{\mathsf{CP}}
\newcommand{\EW}{\mathsf{EW}}
\newcommand{\dd}{\textnormal{d}}

\newcommand{\inD}{   \overset{ \textnormal{d}   }{\rightarrow} }
\newcommand{\inAS}{   \overset{ \textnormal{a.s.}   }{\rightarrow} }
\newcommand{\inP}{  \overset{ \textnormal{pr}    }{\rightarrow} }
\newcommand{\inLp}{ \overset{ \mathcal{L}^p }{\rightarrow} }
\newcommand{\inMSE}{ \overset{ \textnormal{qm} }{\rightarrow} }
\newcommand{\inQM}{ \overset{ \textnormal{qm} }{\rightarrow} }
%\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\indep}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern4mu{#1#2}}}
\newcommand{\eqD}{   \overset{ \text{$\mathcal{D}$}   }{=} }
\newcommand{\iid}{\textsc{iid}} 
\newcommand{\simIID}{   \overset{ \iid   }{\sim} }
\newcommand{\simIND}{   \overset{ {\indep}   }{\sim} }
\newcommand{\simApprox}{   \dot{\sim} }

\newcommand{\Bern}{\textnormal{Bern}} 
\newcommand{\Unif}{\textnormal{Unif}} 
\newcommand{\Normal}{\textnormal{N}} 
\newcommand{\logNormal}{\textnormal{LN}} 
\newcommand{\Bin}{\textnormal{Bin}} 
\newcommand{\NB}{\textnormal{NB}} 
\newcommand{\HG}{\textnormal{HG}} 
\newcommand{\Geom}{\textnormal{Geom}} 
\newcommand{\Beta }{\textnormal{Beta}} 
\newcommand{\BetaBin}{\textnormal{Beta-Bin}}
\newcommand{\Ga}{\textnormal{Ga}} 
\newcommand{\Exp}{\textnormal{Exp}} 
\newcommand{\Expo}{\textnormal{Expo}} 
\newcommand{\Po}{\textnormal{Po}} 
\newcommand{\Multi}{\textnormal{Multi}} 
\newcommand{\student}{\textnormal{t}} 
\newcommand{\Cauchy}{\textnormal{Cauchy}} 
\newcommand{\Pareto}{\textnormal{Pareto}} 
\newcommand{\Laplace}{\textnormal{Laplace}} 
\newcommand{\Logistic}{\textnormal{Logistic}} 
\newcommand{\Dir}{\textnormal{Dir}} 
\newcommand{\DP}{\textnormal{DP}} 
\newcommand{\Inv}{\textnormal{Inv-}} 
\newcommand{\F}{\textnormal{F}} 
\newcommand{\pearson}{\textsc{pc}}
\newcommand{\LR}{\textsc{lr}}
\newcommand{\LLR}{\textsc{llr}}
\newcommand{\spearman}{\textsc{s}}
\newcommand{\AR}{\textnormal{AR}} 
\newcommand{\ARMA}{\textnormal{ARMA}} 
\newcommand{\MA}{\textnormal{MA}} 

\newcommand{\NBM}{\mathop{\mathrm{NBM}}}
\newcommand{\OBM}{\mathop{\mathrm{OBM}}}
\newcommand{\HOC}{\mathop{\mathrm{HOC}}}
\newcommand{\QS}{\mathop{\mathrm{QS}}}
\newcommand{\eff}{\mathop{\mathsf{eff}}}
\newcommand{\diff}{\mathop{\mathsf{diff}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
%\newcommand{\upper}{\mathop{\mathrm{upper}}}
\DeclareMathOperator{\upper}{\mathrm{vech}}
\newcommand{\vectorized}{\mathop{\mathrm{vec}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\rect}{\mathop{\mathsf{rect}}}

\newcommand{\MIT}{\mathsf{MIT}}
\newcommand{\mMIT}{\mathsf{mMIT}}
\newcommand{\MITlong}{\mathsf{long}}
\newcommand{\MITshort}{\mathsf{short}}
\newcommand{\pilot}{\mathsf{pilot}}

\newcommand{\fisher}{\mathsf{fish}}
\newcommand{\one}{\mathsf{one}}
\newcommand{\two}{\mathsf{two}}
\newcommand{\all}{\mathsf{all}} 
\newcommand{\cov}{\mathsf{cov}} 
\newcommand{\trend}{\mathsf{trend}} 
\newcommand{\mix}{\mathsf{mix}} 
\newcommand{\coh}{\mathsf{coh}} 
\newcommand{\fun}{\mathsf{fun}} 
\newcommand{\dcc}{\mathsf{dcc}} 
\newcommand{\noise}{\mathsf{noise}} 


\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\sqw}{sw}
\DeclareMathOperator{\atanh}{atanh}
\def\T{{ \mathrm{\scriptscriptstyle T} }}
%\newcommand{\T}{\textsc{T}}
\newcommand{\comp}{\textsc{c}}

%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### \widecheck
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
%\usepackage{mathabx} %% widecheck 
\usepackage{mathtools}
\makeatletter
\DeclareRobustCommand\widecheck[1]{{\mathpalette\@widecheck{#1}}}
\def\@widecheck#1#2{%
    \setbox\z@\hbox{\m@th$#1#2$}%
    \setbox\tw@\hbox{\m@th$#1%
       \widehat{%
          \vrule\@width\z@\@height\ht\z@
          \vrule\@height\z@\@width\wd\z@}$}%
    \dp\tw@-\ht\z@
    \@tempdima\ht\z@ \advance\@tempdima2\ht\tw@ \divide\@tempdima\thr@@
    \setbox\tw@\hbox{%
       \raise\@tempdima\hbox{\scalebox{1}[-1]{\lower\@tempdima\box
\tw@}}}%
    {\ooalign{\box\tw@ \cr \box\z@}}}
\makeatother

%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### \widebreve
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\makeatletter
\def\widebreve{\mathpalette\wide@breve}
\def\wide@breve#1#2{\sbox\z@{$#1#2$}%
     \mathop{\vbox{\m@th\ialign{##\crcr
\kern0.08em\brevefill#1{0.8\wd\z@}\crcr\noalign{\nointerlineskip}%
                    $\hss#1#2\hss$\crcr}}}\limits}
\def\brevefill#1#2{$\m@th\sbox\tw@{$#1($}%
  \hss\resizebox{#2}{\wd\tw@}{\rotatebox[origin=c]{90}{\upshape(}}\hss$}
\makeatletter



%------------------------------------------
% lty
\usepackage{tikz}
\DeclareRobustCommand\solidLine  {\tikz[baseline=-0.6ex]\draw[thick] (0,0)--(0.5,0);}
\DeclareRobustCommand\dottedLine{\tikz[baseline=-0.6ex]\draw[thick,dotted] (0,0)--(0.54,0);}
\DeclareRobustCommand\dashedLine{\tikz[baseline=-0.6ex]\draw[thick,dashed] (0,0)--(0.54,0);}
\DeclareRobustCommand\dotdashedLine {\tikz[baseline=-0.6ex]\draw[thick,dash dot] (0,0)--(0.5,0);}
%\newcommand{\solidLine}{$\bm{-\!\!\!\!\!-\!\!\!\!\!-\!\!\!\!\!-\!\!\!\!\!-\!\!\!\!\!-\!\!\!\!\!-\!\!\!\!\!-\!\!\!\!\!-}$}
%\newcommand{\dottedLine}{$\bm{\cdot~\cdot~\cdot~\cdot}$}
%\newcommand{\dashedLine}{$\bm{---}$}
%\newcommand{\dotdashedLine}{$\bm{-\cdot-\cdot-}$}


%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%
%%% 
%%% ### marginnote
%%%
%%%----------------------------------------------------------------------------%%%
%%%----------------------------------------------------------------------------%%%	
\usepackage{marginnote}
\newcommand{\note}[1]{\reversemarginpar\marginnote{\scriptsize \color{myred}\!\!\!\!\!\!\!\!\!\!\!\!\!\begin{minipage}{0.15\textwidth}[\textsf{KW:  #1}]\end{minipage}}}
\newcommand{\notealso}[1]{\normalmarginpar\marginnote{\scriptsize \color{myred}\!\!\!\!\!\begin{minipage}{0.15\textwidth}[\textsf{KW:  #1}]\end{minipage}}}
\newcommand{\noteHK}[1]{\reversemarginpar\marginnote{\scriptsize \color{myred}\!\!\!\!\!\!\!\!\!\!\!\!\!\begin{minipage}{0.15\textwidth}[\textsf{HK:  #1}]\end{minipage}}}
\newcommand{\notealsoHK}[1]{\normalmarginpar\marginnote{\scriptsize \color{myred}\!\!\!\!\!\begin{minipage}{0.15\textwidth}[\textsf{HK:  #1}]\end{minipage}}}

\newcommand{\review}{
\begin{center}{\color{BUred}\vspace{2cm}-------------------- \fbox{Reviewed until this point \@~\today}~--------------------\vspace{2cm}}\end{center}}


